A Zero Attentive Relevance Matching Networkfor Review Modeling in Recommendation System

User and item reviews are valuable for the construction of recommender systems. In general, existing review-based methods for recommendation can be broadly categorized into two groups: the siamese models that build static user and item representations from their reviews respectively, and the interaction-based models that encode user and item dynamically according to the similarity or relationships of their reviews. Although the interaction-based models have more model capacity and fit human purchasing behavior better, several problematic model designs and assumptions of the existing interaction-based models lead to its suboptimal performance compared to existing siamese models. In this paper, we identify three problems of the existing interaction-based recommendation models and propose a couple of solutions as well as a new interaction-based model to incorporate review data for rating prediction. Our model implements a relevance matching model with regularized training losses to discover user relevant information from long item reviews, and it also adapts a zero attention strategy to dynamically balance the item-dependent and item-independent information extracted from user reviews. Empirical experiments and case studies on Amazon Product Benchmark datasets show that our model can extract effective and interpretable user/item representations from their reviews and outperforms multiple types of state-of-the-art review-based recommendation models.

==> old.tex <==
\begin{thebibliography}{10}
\bibitem{DeepCoNN}
Lei Zheng, Vahid Noroozi, Philip S. Yu.
\newblock Joint Deep Modeling of Users and Items Using Reviews for
Recommendation
\newblock In {WSDM 2017. 425–434. }

\bibitem{narre}
Chong Chen, Min Zhang, Yiqun Liu, Shaoping Ma. 
\newblock Neural Attentional Rating Regression with Review-level
Explanations.
\newblock In {WWW '18. Pages 1583–1592.}

\bibitem{HANN}
Dawei Cong, anyan Zhao, Bing Qin,
Yu Han, Murray Zhang
\newblock Hierarchical Attention based Neural Network for Explainable Recommendation
\newblock In {CMR ’19, June 10–13, 2019, Ottawa, ON, Canada}

\bibitem{AHN}
Xin Dong, Jingchao Ni, Wei Cheng, Zhengzhang Chen, Bo Zhang, Dongjin Song, Yanchi Liu, Haifeng Chen, Gerarad de Melo
\newblock Asymmetrical Hierarchical Networks with Attentive Interactions for Interpretable Review-Based Recommendation 
\newblock In {AAAI 2020.}

\bibitem{attention}
Ashish Vaswani, Noam Shazeer, Niki Parmar, Jakob Uszkoreit, Llion Jones, Aidan N. Gomez, Łukasz Kaiser, Illia Polosukhin
\newblock Attention Is All You Need
\newblock In {31st Conference on Neural Information Processing Systems (NIPS 2017), Long Beach, CA, USA.}

\bibitem{relative attention}
Peter Shaw, Jakob Uszkoreit, Ashish Vaswani
\newblock Self-Attention with Relative Position Representations
\newblock In {Proceedings of NAACL-HLT 2018, pages 464–468}

\bibitem{cnndlga}
Sungyong Seo, Jing Huang, Hao Yang, Yan liu.
\newblock Interpretable Convolutional Neural Networks with Dual Local and Global Attention for Review Rating Prediction
\newblock In {RecSys '17. 297–305.}

\bibitem{HUITA}
Chuhan Wu, Fangzhao Wu, Junxin Liu, and Yongfeng Huang.
\newblock Hierarchical User and Item Representation with Three-Tier Attention for Recommendation
\newblock In {Proceedings of NAACL-HLT 2019, pages 1818–1826}

\bibitem{mf}
 Y. Koren, R. Bell, and C. Volinsky.
\newblock Matrix factorization techniques for recommender systems
\newblock In {Computer, 42(8), 2009}

\bibitem{MPCN}
Y. Tay, A. T. Luu, and S. C. Hui.
\newblock Multi-pointer co-attention networks for recommendation.
\newblock In { In ACM SIGKDD, 2018.}

\bibitem{fm}
Steffen Rendle.
\newblock Factorization Machines
\newblock In {ICDM '10: Proceedings of the 2010 IEEE International Conference on Data Mining December 2010 Pages 995–1000}

\bibitem{rnn and cnn}
Wenpeng Yin, Katharina Kann, Mo Yu, and Hinrich Schutze. \newblock Comparative study of cnn and rnn for natural
language processing. 
\newblock arXiv preprint arXiv:1702.01923.

\bibitem{googlenews}
Tomas Mikolov, Ilya Sutskever, Kai  Chen, Greg S Corrado, J. Dean 
\newblock Distributed representations of words and phrases and their compositionality
\newblock In {NIPS'13: Proceedings of the 26th International Conference on Neural Information Processing Systems - Volume 2 December 2013 Pages 3111–3119}
%\bibitem{adam}
%D. Kingma, J. Ba. 2014.
%\newblock Adam: A Method for Stochastic Optimization
%\newblock In {arxiv:1412.6980}

\bibitem{amazon dataset}
R. He, J. McAuley
\newblock Ups and downs: Modeling the visual evolution of fashion trends with one-class collaborative filtering
\newblock WWW, 2016

\bibitem{TopicIntegratedHFT}
Julian McAuley and Jure Leskovec
\newblock Hidden factors and hidden topics: understanding rating dimensions with review text
\newblock In RecSys 165–172 2013

\bibitem{TopicIntegratedRMR}
Guang Ling, Michael R Lyu, and Irwin King
\newblock Ratings meet reviews, a combined approach to recommend
\newblock In RecSys 105–112 2014

\bibitem{TopicMF}
Yang Bao, Hui Fang, Jie Zhang
\newblock TopicMF: Simultaneously Exploiting Ratings and Reviews for Recommendation
\newblock In {AAAI 2014, Pages: 2-8}

\bibitem{neurMF}
Xiangnan He, Lizi Liao, Hanwang Zhang, Liqiang Nie, Xia Hu, and Tat-Seng Chua. 
\newblock Neural collaborative filtering.
\newblock In {Proceedings ofthe 26th International Conference on World Wide Web. International World Wide Web Conferences Steering Committee, 173–182.}

\bibitem{NLTK}
Edward Loper , Steven Bird
\newblock NLTK: The Natural Language Toolkit (2002)
\newblock In {ACL'2002}

\bibitem{re2}
Yang, Runqi and Zhang, Jianhai and Gao, Xing and Ji, Feng and Chen, Haiqing
\newblock Simple and Effective Text Matching with Richer Alignment Features
\newblock In {Association for Computational Linguistics (ACL), 2019}

\bibitem{esim}
Chen, Qian and Zhu, Xiaodan and Ling, Zhenhua and Wei, Si and Jiang, Hui and Inkpen, Diana
\newblock Enhanced LSTM for Natural Language Inference
\newblock In {Proceedings of the 55th Annual Meeting of the Association for Computational Linguistics (ACL 2017)}

\bibitem{caffe}
Yi Tay and Luu Anh Tuan and Siu Cheung Hui
\newblock Compare, Compress and Propagate: Enhancing Neural Architectures with Alignment Factorization for Natural Language Inference
\newblock In {Proceedings of EMNLP 2018}
%\bibitem{dropout}
%Nitish Srivastava, imageGeoffrey Hinton, Alex Krizhevsky, Ilya  Sutskever, Ruslan R Salakhutdinov \newblock Dropout: a simple way to prevent neural networks from overfitting
%\newblock In {JMLR'14}

\bibitem{qa-attentive}
Cícero Nogueira dos Santos, Ming Tan, Bing Xiang, and Bowen Zhou
\newblock Attentive Pooling Networks. 
\newblock In {CoRR abs/1602.03609 (2016)}.

\bibitem{drmm}
Jiafeng Guo, Yixing Fan, Qingyao Ai, W. Bruce Croft
\newblock A Deep Relevance Matching Model for Ad-hoc Retrieval
\newblock In {CIKM 2016}

\bibitem{knrm}
Chenyan Xiong, Zhuyun Dai, Jamie Callan, Zhiyuan
Liu, and Russell Power  
\newblock End-to-end neural ad-hoc ranking with kernel pooling. 
\newblock In {In Proceedings of the 40th International ACM SIGIR Conference on Research and Development in Information Retrieval, SIGIR ’17, pages 55–64, Shinjuku, Tokyo,
Japan}

\bibitem{how-review}
Noveen Sachdeva, Julian McAuley
\newblock How Useful are Reviews for Recommendation? A Critical Review and Potential Improvements
\newblock In {SIGIR '20}

\bibitem{ahn}
Xin Dong, Jingchao Ni, Wei Cheng, Zhengzhang Chen, Bo Zong, Dongjin Song, Yanchi Liu, Haifeng Chen, Gerard de Melo
\newblock Asymmetrical Hierarchical Networks with Attentive Interactions for Interpretable Review-Based Recommendation
\newblock In {AAAI 2020}

\bibitem{zero-attention}
Qingyao Ai, Daniel N Hill, SVN Vishwanathan, and W Bruce Croft. 2019. 
\newblock A Zero Attention Model for Personalized Product Search. 
\newblock In {arXiv preprint arXiv:1908.11322
(2019).}

\bibitem{AreWeReallyMakingProgress}
Maurizio Ferrari Dacrema, Paolo Cremonesi, Dietmar Jannach. 2019
\newblock Are We Really Making Much Progress? A Worrying Analysis of Recent Neural Recommendation Approaches
\newblock In {arXiv preprint arXiv:1907.06902 (2019.)}

\bibitem{HowUsefulAreReviews}
Noveen Sachdeva, Julian McAuley
\newblock How Useful are Reviews for Recommendation? A Critical Review and Potential Improvements
\newblock In In {arXiv preprint arXiv:2005.12210 (2020.)}

\end{thebibliography}

==> proposed_method_old.tex <==
\section{Proposed Method}
In this section, we will propose a hybrid interaction-based model based on relevance matching, see int Figure 

We use the relevance matching method to compute the dynamic relevant score of each review of the user to the target. And based on the relevant scores, our model exploits the zero-attention network to decide whether using the dynamic learned target-dependent representations or using static representations for modeling the user. To learn static representations of the user and item, we follow the multi-layer hierarchical paradigms that we learn static user/item representations from their reviews; learn review representations from sentences; and learn sentence representations from words. We first introduce several main components of the model; In section \ref{sec:relmodule}, we introduce the relevance matching module and in section \ref{sec:module}, we introduce the sequence encoding and aggregating modules for static user/item representation modeling. Then in the section \ref{sec:arch} we introduce the overall architecture.

\subsection{Relevance Matching Module} \label{sec:relmodule}
\textbf{\underline{Relevance Matching Module}} treats a user review as a query and the target item reviews as a document, and trains a relevance matching function $m(\cdot, \cdot)$ to check whether the query-document pair is relevant or not. Formally, assumed the $k-th$ user review consists of a sequence of word embeddings $\{ \bm{e}_1^u, \ldots, \bm{e}_l^u \} := \bm{S}_u^k$, and the item document representation consists of a concatenation of a sequence of word embeddings of its each review  $\{ \bm{e}_1^i, \ldots, \bm{e}_l^i, \ldots, \bm{e}_{(m-1)l +1}^i, \ldots, \bm{e}_{ml}^i\} := \bm{S}_i$, where $\bm{e}^u_k, \ \bm{e}^i_k \in \mathbb{R}^d$, $\bm{S}^k_u \in \mathbb{R}^{d \times l}$,  $\bm{S}^i \in \mathbb{R}^{d \times ml}$, $d$ is the dimension of the word embedding, $l$ is the review length, and $m$ is the number of review from the target item. To get the relevant matching score from the $k-th$ user review to its target item, we first compute the word similarity matrix $S$, 
\begin{align}
    \bm{M} = {\bm{S}^k_u}^T \bm{S}_i \in \mathbb{R}^{l \times ml} 
\end{align}
where $\mathbf{M}_{i,j}$ can be considered as similarity score by matching $i-th$ word of user review with $j-th$ word of item document. We apply mean pooling and max pooling on every row of similarity matrix to obtain discriminate features.
\begin{align}
    mean(\mathbf{M}) = \begin{bmatrix} mean(\mathbf{M_{1:}}) \\  \ldots  \\ mean(\mathbf{M_{n:}}) \end{bmatrix} \in \mathbb{R}^l \ , 
    max(\mathbf{M}) = \begin{bmatrix} max(\mathbf{M}_{1:}) \\  \ldots  \\ max(\mathbf{M}_{n:}) \end{bmatrix} \in \mathbb{R}^l
\end{align}
Also, we consider the relative important score for each word in the user review $\bm{S}^k_u$ by applying a function $imp(\cdot)$ , 
\begin{align}
    imp({\mathbf{S}_u^k}) = \begin{bmatrix} 
              imp({\mathbf{e}_1^u}) \\
              \ldots \\
              imp({\mathbf{e}_l^u})
    \end{bmatrix} \in \mathbb{R}^l \ \ \text{where}, \ \
    imp(\bm{e}_j^u) = \frac{\exp({\bm{w}_{p}^T \bm{e}_k^u)}}{\sum_{o=1}^n \exp({\bm{w}_{p}^T} \bm{e}_o^u)}
\end{align}
where $\bm{w}_{p} \in \mathbb{R}^d$, then the input feature for scoring function is \begin{align}
    \bm{I}^{rel} =  \begin{bmatrix} 
        imp(\bm{S}^k_u) \odot mean(\mathbf{M}) \\
        imp(\bm{S}^k_u) \odot  max(\mathbf{M})
    \end{bmatrix} \in \mathbb{R}^{2l}
\end{align}
the scoring function $sg$ is further parameterized by a two layer feed-forward neural network. Hence the relevant score between the $k-th$ user review $\bm{S}^u_k$ and item document $\bm{S}^i$ is,
\begin{align}
    m(\bm{S}^u_k, \bm{S}^i) = sg(\bm{I}^{rel}) = \alpha_k \label{eq:matching}
\end{align}
\subsection{Sequence Encoding \& Aggregating Module} \label{sec:module}
\noindent \textbf{\underline{Sequence Encoding Module}} learns a contextual representation for each element in the sequence by considering the local and global relations between them. It is a stack of a convolution layer, a multihead self-attention layer, and a feed-forward layer.  Formally, the input of the module is a sequence of embeddings $\{ \bm{x_1}, \ldots, \bm{x_t} \}$, and the output is $\{ \bm{z_1}, \ldots, \bm{z_t} \}$, where $\bm{x_i} \in \mathbb{R}^d$, $\bm{z_i} \in \mathbb{R}^{d_k}$, $d$ is the dimension of input embeddings, and $d_k$ is the hidden dimension of the module. First, we use the convolution network to learn n-gram features from the input sequence.  Mathematically, for a sequence of embeddings $\{ \bm{x_1}, \ldots, \bm{x_t} \}$, we denote $\bm{c}_i \in \mathbb{R}^{dn}$ as a concatenation of embeddings $\bm{x}_{i-\lfloor \frac{n-1}{2}\rfloor}, \ldots, \bm{x}_{i+\lfloor \frac{n-1}{2}\rfloor}$, where $n$ is the width. Then we can learn the n-gram feature: $\bm{q}_i$, $\bm{k}_i$, $\bm{v}_i$ from  $\bm{x}_{i-\lfloor \frac{n-1}{2}\rfloor}, \ldots, \bm{x}_{i+\lfloor \frac{n-1}{2}\rfloor} $ by using the convolution weights $\{ \bm{W}_Q, \bm{W}_K, \bm{W}_V \} \in \mathbb{R}^{d_k \times nd}$  and biases $\{ \bm{b}_Q, \bm{b}_K, \bm{b}_V\} \in \mathbb{R}^{d_k}$ respectively: 
\begin{align}
    \bm {q}_i = \text{Relu}(\bm{W}_Q   \bm{c}_i + \bm{b}_Q) ,\
\bm{k}_i = \text{Relu}(\bm{W}_K  \bm{c}_i + \bm{b}_K) ,\
    \bm{v}_i = \text{Relu}(\bm{W}_V  \bm{c}_i + \bm{b}_V)
\end{align}

After the extraction of n-gram features, we take them as input to the multihead self-attention network . We use self-attention since it can capture the long-range dependencies of the sequence which is the complementary to local n-gram feature. Formally, we split $(\bm{q}_i, \bm{k}_i, \bm{v}_i )_{i=1}^t$ into H heads, denoted as $( \bm{q}_i^{h}, \bm{k}_i^{h}, \bm{v}_i^{h} )_{i=1}^t$ for each head, where $\{  \bm{q}_i^{h}, \bm{k}_i^{h}, \bm{v}_i^{h} \} \in \mathbb{R}^{d_h}$ and $d_h$ is the subspace dimension for each head. We apply the same operation to each head. Besides we use relative position embeddings \cite{relative attention} $\bm{p}^V$, $\bm{p}^K$ to encode the pairwise distance between input sequences. Formally, each head's output $\bm{z}_i^{h}$ is the weighted sum of transformed inputs with a learnable vector $\bm{p}_{ij}^V \in R^{d_h}$ encoding the distance between element $i$ and element $j$, 
\begin{equation}\mathbf{z}_i^{h} = \displaystyle\sum_{j=1}^t a_{ij}^{h} (\bm{v}^{h}_j + \bm{p}^V_{ij} ) \label{eq:pos} \end{equation}
each weighted coefficient is computed using a softmax function,
\begin{equation} a_{ij}^{h} = \frac{\exp{(e_{ij}^{h})}}{\sum_{l=1}^t \exp{(e_{il}^{ h}})}\end{equation}

And $e_{ij}^{h}$ is computed as the inner product between two elements,
\begin{equation}e_{ij}^{h} = \frac{<\bm{q}_i^{h}, \bm{k}_j^{h} + \bm{p}^K_{i,j}>}{\sqrt{d_h}}\end{equation}
where $\bm{p}^K_{i,j} \in \mathbb{R}^{d_h}$ is a learnable parameter. Noted that the $\bm{p}^V_{ij}$ and $\bm{p}^K_{i,j}$ are different parameters since one encodes the positional information between values $(\bm{v}_i^h)_{i=1}^t$, and the other encodes the positional information between keys $(\bm{k}_i^h)_{i=1}^t$, but they can be shared across attention heads.
Finally, we concatenate each head's output $\bm{z}_i^{h}$ to get $\bm{z}_i$ and apply a one layer feed-forward network with weights $\bm{W}_f$, bias $\bm{b}_f$ to learn a more flexible representation,
\begin{equation}
    \bm{z}_i = \text{Relu} (\bm{W}_f \bm{z}_i + \bm{b}_f)
\end{equation}
where $\bm{W}_f \in \bb{R}^{d_k \times d_k}$, $\bm{b}_f \in  \bb{R}^{d_k}$. 

\noindent \textbf{\underline{Sequence Aggregating Module}} takes the output of the sequence encoding module as input, and distills their information to form a single vector using attention network. We then treat the vector as the representation of the sequence. Formally, let $\{ \bm{z_1}, \ldots \bm{z_t} \}$ be the input sequence, then the $i-th$ element importance score is computed as,
\begin{align}
    a_i &= \bm{h}^T \text{Relu} (\bm{W}_p \bm{z}_i + \bm{b}_p) \\
    a_i &= \frac{\exp(a_i)}{\sum_{j=1}^t \exp(a_j)}
\end{align}
where $\bm{W}_p \in \mathbb{{R}}^{d_p \times d_k}$, $\bm{b}_p \in \mathbb{R}^{d_p}$, $\bm{h} \in \mathbb{R}^{d_p}$ are learnable parameters, and in our model, we set $d_p = \frac{d_k}{2}$. 
Then the final output $\bm{l}$ is the weighted sum of contextual representations of each element, 
\begin{equation}
    \bm{l} = \displaystyle\sum_{i=1}^t a_i \bm{z}_i \label{eq:aggr}
\end{equation} 
\subsection{Model Architecture} \label{sec:arch}
\textbf{\underline{Sentence Encoder}}. The sentence encoder learns a sentence representation from words, and there are three modules in the encoder.
The first one is a word embedding layer that maps a sequence of words from a sentence to their corresponding dense vectors. Mathematically, assume a sentence $s$ consists of words $\{ w_{1}, \ldots w_{ t}\}$ with size of $t$. The embedding layer transforms the word sequence into dense vectors $\{ \bm{e_1}, \ldots \bm{e_t} \}$, where $\bm{e_i} \in \mathbb{R}^d$. We denote the word embedding matrix as $\mathbf{E} \in \mathbb{R}^{V \times d}$, where $V$ is the word vocabulary size, $d$ is the dense vector dimension. \par 
The second one is a word-level sequence encoding module we defined in section \ref{sec:module}, and we denote it as a function $f_s$. The input of the function is word embeddings $\{ \bm{e_1}, \ldots \bm{e_t} \}$, and the output is their corresponding contextual representations $\{ \bm{z^w_1}, \ldots \bm{z^w_t} \}$, which are computed as,
\begin{equation}
    \{ \bm{z^w_1}, \ldots \bm{z^w_t} \} = f_s (\{\bm{e_1}, \ldots \bm{e_t}\}, d_w)
\end{equation}
where $d_w$ is the hidden dimension of the module, and $\bm{z_i^w} \in \mathbb{R}^{d_w}$. \par 
The third module is a word-level sequence aggregating module defined in section \ref{sec:module}. We denote it as a function $g_s$, and it takes contextual representations $\{ \bm{z^w_1}, \ldots \bm{z^w_t} \}$ as input to get the final sentence embedding, \begin{equation}
    \bm{s} = g_s (\{ \bm{z^w_1}, \ldots \bm{z^w_t} \})
\end{equation}

\noindent \textbf{\underline{Review Encoder}}.
The review encoder learns a review representation from its sentences, which consists of two major modules. The first module is a sentence-level sequence encoding module, and we treat it as a function $f_r$. For each
review, the function takes a sequence of sentence embeddings $\{\bm{s}_1, \ldots \bm{s}_n \}$ as input and get their corresponding contextual representations $\{ \bm{z}^s_1, \ldots \bm{z}^s_n \}$, which are computed as,
\begin{equation}
    \{ \bm{z^s_1}, \ldots \bm{z^s_n} \} = f_r (\{\bm{s_1}, \ldots \bm{s_n}\}, d_s)
\end{equation}
where $d_s$ is the hidden dimension of the the  module, and $\bm{z^s_i}\in \mathbb{R}^{d_s}$.
\par 
The second module of the review encoder is the sentence-level aggregating module, and we denote it as $g_r$. The input of the function is $\{ \bm{z}^s_1, \ldots \bm{z}^s_n \}$, and the output is the review representation $r$, 
\begin{equation}
    \bm{r} = g_r (\{ \bm{z^s_1}, \ldots \bm{z^s_n} \})
\end{equation}

\noindent \textbf{\underline{User/Item Encoder}}.
We learn a user and item representations using review-level aggregating module, denoted as $g_u, \ g_i$, to select their reviews with more informativeness. Formally, we assume a user $u$ writes $m$ reviews,
$\bm{r}^u_1, \ldots \bm{r}_m^u$, and item $i$ has $m$ reviews, $\bm{r}^i_1, \ldots \bm{r}_m^i$ and  then the final static user and item representation can be computed as,
\begin{align}
    \bm{u}^{static} &= g_u ( \bm{r}^u_1, \ldots \bm{r}_m^u ) \\ 
    \bm{i}^{static} &= g_i ( \bm{r}^i_1, \ldots \bm{r}_m^i )
\end{align}
Each user and item reviews can be represented by sequence of word embeddings alternatively. Hence the word sequence representations of user is $\{ \bm{S}^u_1, \ldots \bm{S}^u_m \}$, and the item is   
$\{ \bm{S}^i_1, \ldots \bm{S}^i_m \}$, where $\bm{S}^*_* \in \mathbb{R}^{d \times l}$, $d$ is the word embedding dimension, $l$ is the number of word in each review. We concatenate the item reviews as a item document $[ \bm{S}^i_1, \ldots \bm{S}^i_m ] := \bm{S}^i \in \mathbb{R}^{d \times ml}$, then we compute the dynamic relevance matching score between the $k-th$ user review with the target item document using the Equation \ref{eq:matching},
\begin{align}
    \alpha_k = m(\bm{S}^u_k, \bm{S}^i) \in [-\infty, \infty]
\end{align}
We rescale the relevance matching score using the zero-attention technique [1], $\hat{\alpha}_k = \frac{1 + \exp(\alpha_k)}{1 + \exp{(\alpha_1)} + \ldots \exp{(\alpha_m)}}, \ k=1, \ldots m$, and $\hat{\alpha}_0 = \frac{1}{1 + \exp{(\alpha_1)} + \ldots \exp{(\alpha_m)}}$, then the user dynamic representation is,
\begin{align}
    \mathbf{u}^{dynamic} &= \displaystyle\sum_{k=1}^m \hat{\alpha}_k \mathbf{r_k} + \hat{\alpha_0} \vec{\mathbf{0}} 
\end{align}
the final user, item representation from reviews is,
\begin{align}
    \bm{u}^r &= \text{Relu} \Big( \begin{bmatrix} 
    \mathbf{W}^{static}_u, & \mathbf{W}^{dynamic}_u
     \end{bmatrix}\begin{bmatrix}
        \bm{u}^{static} \label{eq:u} \\
        \bm{u}^{dynamic} 
        \end{bmatrix}  + \mathbf{b}_u \Big) \\ 
    \bm{i}^r &= \text{Relu} \Big(  \bm{W}^{static}_i \bm{i}^{static} + \mathbf{b}_i \Big) \label{eq:i}
\end{align}
, where $\bm{W}^{static}_u, \ \bm{W}^{static}_u ,\ \bm{W}^{dynamic}_i, \ \bm{W}^{static}_i \in \mathbb{R}^{d_h \times d_s}$, $\bm{b}_u, \ \bm{b}_i \in \mathbb{R}^{d_h}$. \\
Intuitively, when there is not dynamic relevant matching signal between user reviews to the target item, all $\hat{\alpha}_k, \ k = 1, \ldots m$ will be close to $0$, and $\hat{\alpha}_0$ will be close to $0$, then the final user representation will degrade to $\bm{u} = \text{Relu} \big( \mathbf{W}^{static}_u \bm{u}^{static} + \bm{b}_u \big)$. And when there is a valid strong matching signal, the user representation will become $\bm{u} = \text{Relu} \big( \mathbf{W}^{dynamic}_u \bm{u}^{dynamic} + \bm{b}_u \big)$.

\noindent \textbf{\underline{Prediction Layer}}. Given the learned user, item representations from Equation \ref{eq:u}, \ref{eq:i}. Also, we get the corresponding id embedding of the user and item, which is $\bm{u}^{id}$, $\bm{i}^{id} \in \mathbb{R}^{d_h}$, Then the final user, and item representations are $\bm{u} = \bm{u}^r + \bm{u}^{id} ,\ \bm{i} = \bm{i}^r + \bm{i}^{id}$. The final predicted rating prediction is,
\begin{align}
    \hat{y}_{u,i} = \bm{w}_f^T (\bm{u} \odot \bm{i}) + b_u + b_i + b_g \label{eq:rating} 
\end{align}
where $\bm{w}_f \in \mathbb{R}^{d_h}, \ b_u, \ b_i, \ b_g \in \mathbb{R}$ 

\subsection{Training}
We exploit a multitask learning framework to jointly train a regression loss for the rating prediction task and a classification loss for the relevance matching task. Specifically, we assumed there are user-item pair $(u, i)$ with the \textit{ground-truth} rating $y_{u,i}$ in the training stage. In the training stage we can see the \textit{ground-truth} review $r_{u,i}^g$ written from the user to the target item, we view it as a "positive query" to the target item, and also we randomly sample a review from the different user different item as a "negative query" to the target item $r_{u,i}^n$. We let the word sequence representation of the \textit{ground-truth} review, negative review and target item document as $\bm{S}^u_g, \ \bm{S}^u_n, \ \bm{S}^i$, and the predicted rating for each (u,i) pair from the Equation \ref{eq:rating}, then the training objective is,
\begin{align}
     loss = \displaystyle\sum_{\{ (u,i)\} \in \mathcal{S}} \underbrace{\bigg( y_{u,i} - \hat{y}_{u,i} \bigg)^2}_{\text{regression loss}} - \underbrace{\bigg( \log\big( m (\bm{S}^u_g,  \bm{S}^i)\big)- \log\big(1 - m(\bm{S}^u_n,\bm{S}^i) \big)\bigg)}_{\text{classification loss}} \label{eq:loss}
\end{align}
where the $m(\cdot, \cdot)$ is defined in the Equation \ref{eq:matching}, and $\mathcal{S}$ is the set of the user-item pair in the training set.

==> proposed_method_old_v1.tex <==
\section{Proposed Method}
We introduce our proposed model using layer-by-layer description. The overall model can be seen in Figure \ref{fig:arch} \par
\begin{figure}
   \centering
    \includegraphics[width=0.95\textwidth, height=0.65\textwidth]{figures/arch_v2_75.png}
    \caption{Overview of our model structure}
   \label{fig:arch}
\end{figure}
\subsection{Review Encoder} Assume each user and item have $N$ reviews, $\{r^u_1, \ldots r^u_N \}$, $\{r^i_1, \ldots r^i_N \}$, we first encode each review into its own vector representation. We learn a review representation hierarchically from word-level to sentence-level. Given a user review $r^u = \{s_1, \ldots s_T\}$ consists of $T$ sentences, and each sentence $s_i$ is composed of a sequence of $L$ words $ \{w^i_1, \ldots w^i_L \}$. We first apply the word embedding layer to map each word $w^i_j$ into a vector $\bm{w}^i_j \in \mathbb{R}^{d_w}$. Then we use the \textbf{\textit{word-level sequence encoding module}} to learn the semantic feature of each word. The learned semantic features will be taken as inputs to the the \textbf{\textit{word-level aggregating module}} to represent the sentence $s_i$ as a vector $\bm{s}_i \in \mathbb{R}^{d_s}$. Similarly, we use \textbf{\textit{sentence-level sequence encoding module}} to learn contextual feature of each sentence, and aggregate the features using a \textbf{\textit{sentence-level sequence aggregating module}} to form the the review final representation $\bm{r}^u \in \mathbb{R}^{d_r}$. Where $d_w$, $d_s$, $d_r$ is the dimension of word embedding, sentence hidden vector and review hidden vector. In the following of the section, we will introduce these modules in details.

\subsubsection{Word-level Sequence Encoding Module}
The module can be viewed as self-attentive convolution neural network, which is a stack of a convolution layer, a multihead-self-attention layer and a feed-forward layer. The input of the module is $\{ \bm{w}^i_1, \ldots, \bm{w}^i_L \}$, and the output is $\{ \bm{z}^i_1, \ldots, \bm{z}^i_L \}$, where $\bm{w}^i_j \in \mathbb{R}^{d_w}$, $\bm{z}_j^i \in \mathbb{R}^{d_{s}}$. First, we use the convolution network to learn n-gram features from the input sequence.  Mathematically, given the word embeddings $\{ \bm{w}^i_1, \ldots, \bm{w}^i_L \}$, we denote $\bm{c}_j^i \in \mathbb{R}^{nd_w}$ as a concatenation of the embeddings $\bm{w}_{j-\lfloor \frac{n-1}{2}\rfloor}^i, \ldots, \bm{w}_{j+\lfloor \frac{n-1}{2}\rfloor}^i$, where $n$ is the width. Then we can learn the n-gram feature: $\bm{q}_j^i$, $\bm{k}_j^i$, $\bm{v}_j^i$ from  $\bm{w}_{i-\lfloor \frac{n-1}{2}\rfloor}, \ldots, \bm{w}_{i+\lfloor \frac{n-1}{2}\rfloor} $ by using the convolution weights $\{ \bm{W}_Q, \bm{W}_K, \bm{W}_V \} \in \mathbb{R}^{d_s \times nd_w}$  and biases $\{ \bm{b}_Q, \bm{b}_K, \bm{b}_V\} \in \mathbb{R}^{d_s}$ respectively: 
\begin{align}
    \bm {q}_j^i = \text{Relu}(\bm{W}_Q   \bm{c}_j^i + \bm{b}_Q) ,\
\bm{k}_j^i = \text{Relu}(\bm{W}_K  \bm{c}_j^i + \bm{b}_K) ,\
    \bm{v}_j^i = \text{Relu}(\bm{W}_V  \bm{c}_j^i + \bm{b}_V)
\end{align} 
After the extraction of n-gram features, we take them as input to the multihead self-attention network . We use self-attention since it can capture the long-range dependencies of the sequence which is the complementary to local n-gram feature. Formally, we split $(\bm{q}_j^i, \bm{k}_j^i, \bm{v}_j^i )_{j=1}^L$ into H heads, denoted as $( \bm{q}_j^{i,h}, \bm{k}_j^{i,h}, \bm{v}_j^{i, h} )_{j=1}^L$ for each head, where $\{  \bm{q}_j^{i,h}, \bm{k}_j^{i,h}, \bm{v}_j^{i,h} \} \in \mathbb{R}^{d_h}$ and $d_h$ is the subspace dimension for each head. We apply the same operation to each head. Besides we use relative position embeddings \cite{relative-attention} $\bm{p}^V$, $\bm{p}^K$ to encode the pairwise distance between input sequences. Formally, each head's output $\bm{z}_j^{i,h}$ is the weighted sum of transformed inputs with a learnable vector $\bm{p}_{jk}^V \in R^{d_h}$ encoding the distance between element $j$ and element $k$, 
\begin{equation}\mathbf{z}_j^{i,h} = \displaystyle\sum_{j=1}^L a_{jk}^{i,h} (\bm{v}^{i,h}_k + \bm{p}^V_{jk} ) \label{eq:pos} \end{equation}
each weighted coefficient is computed using a softmax function,
\begin{equation} a_{jk}^{i,h} = \frac{\exp{(e_{jk}^{i,h})}}{\sum_{l=1}^L \exp{(e_{jl}^{i,h}})}\end{equation}

And $e_{jk}^{i,h}$ is computed as the inner product between two elements,
\begin{equation}e_{jk}^{i,h} = \frac{<\bm{q}_j^{i,h}, \bm{k}_k^{i,h} + \bm{p}^K_{jk}>}{\sqrt{d_h}}\end{equation}
where $\bm{p}^K_{jk} \in \mathbb{R}^{d_h}$ is a learnable parameter. Noted that the $\bm{p}^V_{ij}$ and $\bm{p}^K_{jk}$ are different parameters since one encodes the positional information between values $(\bm{v}_j^{i,h})_{j=1}^T$, and the other encodes the positional information between keys $(\bm{k}_j^{i,h})_{j=1}^T$, but they can be shared across attention heads.
Finally, we concatenate each head's output $\bm{z}_j^{i,h}$ to get $\bm{z}^i_j$ and apply a one layer feed-forward network with weights $\bm{W}_f$, bias $\bm{b}_f$ to learn a more flexible representation,
\begin{equation}
    \bm{z}^i_j = \text{Relu} (\bm{W}_f \bm{z}^i_j + \bm{b}_f)
\end{equation}
where $\bm{W}_f \in \bb{R}^{d_s \times d_s}$, $\bm{b}_f \in  \bb{R}^{d_s}$.  

\subsubsection{Word-level Aggregating Module}
The module takes the output of the sequence encoding module $\{\bm{z}^i_1 \ldots \bm{z}^i_L \}$ as a input, and distills their information to form a single vector using attention network. We then treat the vector as the representation of the sequence. Formally, the $j-th$ word importance score is computed as,
\begin{align}
    a_j^i &= \bm{h}^T \text{Relu} (\bm{W}_p \bm{z}_j^i + \bm{b}_p) \\
    a_j^i &= \frac{\exp(a_j^i)}{\sum_{l=1}^L \exp(a_j^i)}
\end{align}
where $\bm{W}_p \in \mathbb{{R}}^{\frac{d_s}{2} \times d_s}$, $\bm{b}_p \in \mathbb{R}^{\frac{d_s}{2}}$, $\bm{h} \in \mathbb{R}^{\frac{d_s}{2}}$ are learnable parameters. Then the $i-th$ sentence representation $\bm{s}_i$ is the weighted sum of contextual representations of contextual representation of each word,
\begin{equation}
    \bm{s}_i = \displaystyle\sum_{l=1}^L a_l^i \bm{z}_l^i 
\end{equation} 

\subsubsection{Sentence-level Sequence Encoding Module}
For the sentences $\{s_1, \ldots s_T \}$, we follow the above procedure to learn their vector representations $\{\bm{s}_1, \ldots \bm{s}_T \}$. We take the sentence sequence embeddings as input to the sentence-level sequence module which has the same architecture as word-level sequence module but use the new learned parameters. Then the output of the module is learned sentence contextual embeddings $\{\bm{g}_1, \ldots \bm{g}_T \}$, where $\bm{g}_j \in \mathbb{R}^{d_r}$.

\subsubsection{Sentence-level Aggregating Module}
The module takes the outputs of sentence-level sequence encoding module $\{\bm{g}_1, \ldots \bm{g}_T \}$ as a input into the sentence-level sequence module which has the same architecture as word-level aggregating module but exploits different learnable parameters, and the output of the module is the review representation $\bm{r}^u$. 

\subsection{Static Review Aggregator}
After encoding the user and item review representations $\{\bm{r
}^u_1, \ldots \bm{r}^u_N \}$, $\{\bm{r
}^i_1, \ldots \bm{r}^i_N \}$. We encode the user and item static representation using the attention neural network. We first compute the informativeness score of each user and item review,
\begin{align}
    \hat{b}_j^u &= \bm{h}_u^T \text{Relu} (\bm{W}_p^u \bm{r}_j^u + \bm{b}_p^u) ,\ \ \hat{b}_j^i = \bm{h}_i^T \text{Relu} (\bm{W}_p^i \bm{r}_j^i + \bm{b}_p^i) \\
    b_j^u &= \frac{\exp(\hat{b}_j^u)}{\sum_{l=1}^L \exp(\hat{b}_j^u)} , \ \ b_j^i = \frac{\exp(\hat{b}_j^i)}{\sum_{l=1}^L \exp(\hat{b}_j^i)}
\end{align}
Then the static user and item can be represented as,
\begin{align}
    \bm{u}^{static} &= \displaystyle\sum_{l=1}^N b_l^u \bm{r}_l^u , \ \ 
    \bm{i}^{static} = \displaystyle\sum_{l=1}^N b_l^i \bm{r}_l^i \label{eq:aggr}
\end{align}

\subsection{Relevance Matching Module}
This module learns a user dynamic representation $\bm{u}^{dynamic}$. The module treats a user review as a query and the target item reviews as a document, and trains a relevance matching function $m(\cdot, \cdot)$ to check whether the query-document pair is relevant or not. Formally, we alternatively represent the $k$-th user review as a sequence of word embeddings  $\{ \bm{e}_1^u, \ldots, \bm{e}_M^u \} := \bm{S}_u^k$, and the item document is a concatenation of a sequence of word embeddings of its each review  $\{ \bm{e}_1^i, \ldots, \bm{e}_M^i, \ldots, \bm{e}_{(N-1)M +1}^i, \ldots, \bm{e}_{NM}^i\} := \bm{S}_i$, where $\bm{e}^u_k, \ \bm{e}^i_k \in \mathbb{R}^{d_w}$, $\bm{S}^k_u \in \mathbb{R}^{d_w \times M}$,  $\bm{S}^i \in \mathbb{R}^{d_w \times MN}$, $d_w$ is the dimension of the word embedding, $M$ is the review length, and $N$ is the number of review from the target item. To get the relevant matching score from the $j$-th user review to its target item, we first compute the word similarity matrix $S$, 
\begin{align}
    \bm{M} = {\bm{S}^k_u}^T \bm{S}_i \in \mathbb{R}^{M \times MN} 
\end{align}
where $\mathbf{M}_{i,j}$ can be considered as similarity score by matching $i$-th word of user review with $j$-th word of item document. We apply mean pooling and max pooling on every row of similarity matrix to obtain discriminate features.
\begin{align}
    mean(\mathbf{M}) = \begin{bmatrix} mean(\mathbf{M_{1:}}) \\  \ldots  \\ mean(\mathbf{M_{n:}}) \end{bmatrix} \in \mathbb{R}^M \ , 
    max(\mathbf{M}) = \begin{bmatrix} max(\mathbf{M}_{1:}) \\  \ldots  \\ max(\mathbf{M}_{n:}) \end{bmatrix} \in \mathbb{R}^M
\end{align}
Also, we consider the relative important score for each word in the user review $\bm{S}^k_u$ by applying a function $imp(\cdot)$ , 
\begin{align}
    imp({\mathbf{S}_u^k}) = \begin{bmatrix} 
              imp({\mathbf{e}_l^u}) \\
              \ldots \\
              imp({\mathbf{e}_l^u})
    \end{bmatrix} \in \mathbb{R}^M \ \ \text{where}, \ \
    imp(\bm{e}_j^u) = \frac{\exp({\bm{w}_{p}^T \bm{e}_k^u)}}{\sum_{o=1}^n \exp({\bm{w}_{p}^T} \bm{e}_o^u)}
\end{align}
where $\bm{w}_{p} \in \mathbb{R}^{d_w}$, then the input feature for scoring function is \begin{align}
    \bm{I}^{rel} =  \begin{bmatrix} 
        imp(\bm{S}^k_u) \odot mean(\mathbf{M}) \\
        imp(\bm{S}^k_u) \odot  max(\mathbf{M})
    \end{bmatrix} \in \mathbb{R}^{2M}
\end{align}
the scoring function $sg$ is further parameterized by a two layer feed-forward neural network. Hence the relevant score between the $k$-th user review $\bm{S}^u_k$ and item document $\bm{S}^i$ is,
\begin{align}
    m(\bm{S}^u_k, \bm{S}^i) = sg(\bm{I}^{rel}) = \alpha_k \in [-\infty, \infty] \label{eq:matching} 
\end{align}

\subsubsection{User Dynamic Representation Learning}
After computing the relevance matching score from the user reviews to her target item, $\{\alpha_1, \ldots \alpha_N \}$, we rescale the relevance matching score using the zero-attention technique \cite{zero-attention},\\ $\hat{\alpha}_k = \frac{1 + \exp(\alpha_k)}{1 + \exp{(\alpha_1)} + \ldots \exp{(\alpha_m)}}, \ k=1, \ldots m$, and $\hat{\alpha}_0 = \frac{1}{1 + \exp{(\alpha_1)} + \ldots \exp{(\alpha_m)}}$, then the user dynamic representation is,
\begin{align}
    \mathbf{u}^{dynamic} &= \displaystyle\sum_{k=1}^m \hat{\alpha}_k \mathbf{r_k} + \hat{\alpha_0} \vec{\mathbf{0}} 
\end{align}
Intuitively, when each user review is not relevant to the target item, each rescaled relevance matching score $\hat{\alpha}_k$ will be close to $0$, then the $\bm{u}^{dynamic}$ will degrade to zero vector.

\subsection{Feature Transform Layer}
This layer combine the static and dynamic user to form a final user representation learned from reviews. Also, it learns a final item static representation from reviews by $1$-layer feed-forward neural network,
\begin{align}
    \bm{u}^r &= \text{Relu} \Big( \begin{bmatrix} 
    \mathbf{W}^{static}_u, & \mathbf{W}^{dynamic}_u
     \end{bmatrix}\begin{bmatrix}
        \bm{u}^{static} \label{eq:u} \\
        \bm{u}^{dynamic} 
        \end{bmatrix}  + \mathbf{b}_u \Big) \\ 
    \bm{i}^r &= \text{Relu} \Big(  \bm{W}^{static}_i \bm{i}^{static} + \mathbf{b}_i \Big) \label{eq:i}
\end{align}
, where $\bm{W}^{static}_u, \ \bm{W}^{static}_u ,\ \bm{W}^{dynamic}_i, \ \bm{W}^{static}_i \in \mathbb{R}^{d_h \times d_r}$, $\bm{b}_u, \ \bm{b}_i \in \mathbb{R}^{d_h}$.

\subsection{Prediction Layer}
Given the learned user, item representations from Equation \ref{eq:u}, \ref{eq:i}. Also, we get the corresponding id embedding of the user and item, which is $\bm{u}^{id}$, $\bm{i}^{id} \in \mathbb{R}^{d_h}$, Then the final user, and item representations are $\bm{u} = \bm{u}^r + \bm{u}^{id} ,\ \bm{i} = \bm{i}^r + \bm{i}^{id}$. The final predicted rating prediction is,
\begin{align}
    \hat{y}_{u,i} = \bm{w}_f^T (\bm{u} \odot \bm{i}) + b_u + b_i + b_g \label{eq:rating} 
\end{align}
where $\bm{w}_f \in \mathbb{R}^{d_h}, \ b_u, \ b_i, \ b_g \in \mathbb{R}$ 

\subsection{Training}
We exploit a multitask learning framework to jointly train a regression loss for the rating prediction task and a classification loss for the relevance matching task. Specifically, we assumed there are user-item pair $(u, i)$ with the \textit{ground-truth} rating $y_{u,i}$ in the training stage. In the training stage we can see the \textit{ground-truth} review $r_{u,i}^g$ written from the user to the target item, we view it as a "positive query" to the target item, and also we randomly sample a review from the different user different item as a "negative query" to the target item $r_{u,i}^n$. We let the word sequence representation of the \textit{ground-truth} review, negative review and target item document as $\bm{S}^u_g, \ \bm{S}^u_n, \ \bm{S}^i$, and the predicted rating for each (u,i) pair from the Equation \ref{eq:rating}, then the training objective is,
\begin{align}
     loss = \displaystyle\sum_{\{ (u,i)\} \in \mathcal{S}} \underbrace{\bigg( y_{u,i} - \hat{y}_{u,i} \bigg)^2}_{\text{regression loss}} - \underbrace{\bigg( \log\big( m (\bm{S}^u_g,  \bm{S}^i)\big)- \log\big(1 - m(\bm{S}^u_n,\bm{S}^i) \big)\bigg)}_{\text{classification loss}} \label{eq:loss}
\end{align}
where the $m(\cdot, \cdot)$ is defined in the Equation \ref{eq:matching}, and $\mathcal{S}$ is the set of the user-item pair in the training set.
